The Impact of Neural Network Overparameterization on Gradient Confusion and Stochastic Gradient Descent

This paper studies how neural network architecture affects the speed of training. We introduce a simple concept called gradient confusion to help formally analyze this. When gradient confusion is high, stochastic gradients produced by different data samples may be negatively correlated, slowing down convergence. But when gradient confusion is low, data samples interact harmoniously, and training proceeds quickly. Through theoretical and experimental results, we demonstrate how the neural network architecture affects gradient confusion, and thus the efficiency of training. Our results show that, for popular initialization techniques, increasing the width of neural networks leads to lower gradient confusion, and thus faster model training. On the other hand, increasing the depth of neural networks has the opposite effect. Our results indicate that alternate initialization techniques or networks using both batch normalization and skip connections help reduce the training burden of very deep networks.

==> background.tex <==
%!TEX root = main.tex
\section{Discussion and related work}

For this reason, the optimization community has sought faster methods with better convergence rates for solving classical convex learning problems.  This includes variance reduction methods \cite{johnson2013accelerating, defazio2014saga, schmidt2017minimizing, de2016efficient}, methods that switch from stochastic to deterministic gradient methods when approaching a minimizer \tom{Cite AllReduce paper}, and methods that dynamically increase the batch size to reduce gradient noise \cite{de2016big, friedlander2012hybrid, byrd2012sample, smith2017don}.  

Interpolation paper: \cite{ma2017power}.

\subsection{Theory on constant step-size SGD}

\url{http://tongzhang-ml.org/papers/icml04-stograd.pdf}

\url{http://proceedings.mlr.press/v84/chee18a/chee18a.pdf}

\url{http://proceedings.mlr.press/v84/lakshminarayanan18a/lakshminarayanan18a.pdf}

\subsection{Papers on how over-parameterization affects neural nets}

\cite{arora2018optimization} show that SGD on over-parameterized linear neural nets is similar to applying a certain preconditioner while optimizing.  

\url{https://arxiv.org/pdf/1802.06509.pdf}


\cite{cooper2018loss} Studies the loss surfaces of over-parameterized nets, and shows that they contain high-dimensional manifolds of solutions.
\url{https://arxiv.org/pdf/1804.10200.pdf}

\cite{ma2017power}  Investigate how different learning rates and batch size choices affect convergence of SGD on high-dimensional problems.
\url{https://arxiv.org/pdf/1712.06559.pdf}

\cite{sagun2017empirical} Investigate the Hessian of over-parameterized networks.
\url{https://arxiv.org/abs/1706.04454}

\url{https://arxiv.org/abs/1702.08591}



==> conclusion.tex <==
%!TEX root = main.tex
\section{Discussion}  %, limitations and future work}
%\section{Discussion}
% \vspace{-2mm}

In this paper, we study how neural net architecture affects the dynamics of SGD. To formally analyze this, we introduce a concept called gradient confusion, and show that when gradient confusion is low, SGD has fast convergence. Further, at standard initializations, increasing layer width leads to lower gradient confusion, making the model easier to train. In contrast, increasing depth results in higher gradient confusion, making models harder to train. Finally, we show how the combination of batch normalization and skip connections help train very deep models.

Our results provide a number of important insights that can be used for better neural net model and algorithm design.
%, as well as for better algorithms for better training and generalization. 
Test set accuracies shown in appendix \ref{app:extra_results} suggest that an interesting topic for future work would be to investigate the connection between gradient confusion and generalization \citep{fort2019stiffness}. 
%The difference in the gradient confusion within the same class and across classes could also be an interesting tool to study adversarial training.
Note that many previous results have shown how deeper models are more efficient at modeling higher complexity function classes than wider models, and thus depth is essential for the success of neural nets \citep{eldan2016power, telgarsky2016benefits}. Our results indicate that, given a sufficiently deep net, increasing the network width is important for the trainability of the model, and will lead to faster convergence. This is supported by other recent research \citep{hanin2018neural, hanin2018start} that suggest that the width should increase linearly with depth in a neural net to help dynamics at the beginning of training. Our results also suggest the importance of further investigation into good initialization schemes for neural nets that make training very deep models possible \citep{zhang2019fixup}.

%We consider the main limitation of this work to be the use of the random dataset that consists of i.i.d.~samples of isoperimetric vectors to derive the concentration bounds in Section \ref{sec:syntheticData}. Note that while this simple data model helps make the analysis tractable and gives insights into the effect of overparameterization, it is not clear to what extent real-world datasets follow such a model (\emph{i.e.,} i.i.d.~data and isoperimetric property in the feature space). Nonetheless, these are standard assumptions used in statistical learning theory since it allows for mathematical analysis. To make our observations on this model robust, we show that the same qualitative results hold (i) with arbitrary data and random weights in Section \ref{sec:init} (i.e., at initialization), and (ii) in the experimental setting (Section \ref{sec:experiments} and Appendix \ref{app:mnist}). For future work, it would be interesting to extend this analysis to richer random data models. It would also be interesting to gain a better understanding of how layer width impacts long-term training dynamics, while the analysis here focuses on behavior near initialization.

%An active area of research currently is to better understand how overparameterization and neural net architecture promote generalization \cite{neyshabur2018towards, allen2018learning, belkin2018reconciling, neal2018modern}. An interesting topic for future work is whether there is a connection between gradient confusion, sharp and flat minimizers, and generalization for SGD. See \cite{fort2019stiffness} for some recent work in this direction.

%\soham{Will add a note on the limitations of the results in this paper and possible extensions of these results.}

%==========
%==========
%memorization effect with increasing width; refer to emails.

% more work into initialization of deep networks.

% justify random data model.
%==========
%==========



%\soham{Limitations of proven results}
%
%\soham{Other unrelated places where gradient similarity can be useful: \cite{du2018adapting}.
%
%Also look at predictor of generalization (or cross-validation error) or generating automatic stopping conditions.}
%A related issue is that stochastic noise during training leads to improved generalization performance because of implicit regularization.  This is not our main focus -- we addresses the question of why SGD is good for optimization, rather than why it's good for generalization.    
%
%\soham{Effect of large batches (refer to gradient diversity), effect of momentum. A closer study of the SGD path dynamics.}



==> generalNN.tex <==
%!TEX root = main.tex
Formally, let $\vec{W}_0 \in \mathbb{R}^{\ell_1 \times d}$ and $\{ \vec{W}_p \}_{p \in [\beta]}$ such that $\vec{W}_p \in \mathbb{R}^{\ell_p \times \ell_{p-1}}$ be the given weight matrices. Let $\vec{W}$ denote the tuple $(\vec{W}_p)_{p \in [\beta]_0}$. Define $\ell := \max_{p \in [\beta]} \ell_p$ to be the \emph{width} and $\beta$ to be the \emph{depth} of the neural network. Then, the model $g_{\vec{W}}$ is defined as 
		\begin{equation}
			\label{eq:NNmodel}
			g_{\vec{W}}(\vec{x}) := \sigma(\vec{W}_{\beta} \sigma(\vec{W}_{\beta-1} \ldots \sigma(\vec{W}_1 \sigma(\vec{W}_0 \vec{x}))\ldots )),
		\end{equation}
		where $\sigma$ denotes the non-linear activation function applied point-wise to its arguments. We assume that the non-linear activation is given by a function $\sigma(x)$ with the following properties. 
		\begin{itemize}
			\item \textbf{(P1) Boundedness:} $|\sigma(x)| \leq 1$ for vector $x \in [-1, 1]$.
			\item \textbf{(P2) Bounded differentials:}  Let $\sigma'(x)$ and $\sigma''(x)$ denote the first and second sub-differentials respectively. Then, $|\sigma'(x)| \leq 1$ and $ |\sigma''(x)| \leq 1$ for all $x \in [-1, 1]$.
		\end{itemize}
		When $\|\vec{x}\| \leq 1$, as in our random data model, activation functions such as \emph{sigmoid}, \emph{tanh}, \emph{softmax} and \emph{ReLU} satisfy these requirements. Additionally, we make the following assumption on the weights. \vspace{2mm}

			\begin{assumption}[Small Weights]
				\label{ass:small_weight}
					We assume that the operator norm of the weight matrices $\{\vec{W}_i\}_{i \in [\beta]_{0}}$ are bounded above by $1$. In other words, for every $i \in [\beta]_{0}$ we have $\|\vec{W}_i\| \leq 1$.
				\end{assumption}

%
   		
% \paragraph{Is the small-weights assumption reasonable?} 
 % If we relax the assumption and let every entry in each of the weight matrices lie in the range $[-1, 1],$  then a product of matrices $\vec{W}_\beta \cdot \vec{W}_{\beta-1} \cdot \ldots (\vec{W}_{\beta'})_{k_{\beta'}}$ may lead to an exponential blow up in values. If we have vectors $\vec{v}_1, \vec{v}_2 \in [-1, 1]^{\ell}$ then $\langle \vec{v}_1, \vec{v}_2 \rangle$ can be as large as $\ell$. Hence in a sequence of $\beta$ products of matrices, the final value can become as large as $\ell^\beta$.
The operator norm of the weight matrices $\| \vW \|$ being close to 1 is important for the trainability of neural nets, as it ensures that the input signal is passed through the net without exploding or shrinking across layers \citep{glorot2010understanding}. Proving non-vacuous bounds in case of such blow-ups in magnitude of the signal or the gradient is not possible in general, and thus, we consider this restricted class of weights. The small-weights assumption is not just a theoretical concern, but also usually enforced in practice using \emph{weight decay} regularizers of the form $\sum_i \|W_i\|_F^2$, which keep the weights small during optimization.   See appendix \ref{app:small_weights} for further discussion on the small weights assumption.
% 	
%		The small weights assumption is not just a theoretical concern, but also usually mandated in practice. Without small weights, the gradients $\nabla_{\vec{W}} f_i$ blows up in magnitude and a phenomenon known as \emph{gradient-explosion} (which is particularly problematic for recurrent neural networks) is observed. This may indicate why weights are typically initialized as $\mathcal{N}(0, 1/\ell_i)$ in practice~\citep{bengio2012practical}. 
%
%Note that the small-weights assumption is not just a theoretical concern, but also usually mandated in practice. Neural networks are often trained with \emph{weight decay} regularizers of the form $\sum_i \|W_i\|_F^2$, which force the weights to remain small during optimization.
%The operator norm of convolutional layers have also recently been used as an effective regularizer as well for image classification tasks \citep{sedghi2018singular}. 
		%
%  \xhdr{Assumption~\ref{ass:small_weight} holds for random initialization.} 
%  We can also show formally that Assumption \ref{ass:small_weight} holds with high probability for random initializations that are frequently used in practice \citep{bengio2012practical}.
%  Consider a random weight matrix $\vec{W} \in \mathbb{R}^{\ell_1 \times \ell_2}$ where every entry is an independent sample from $\mathcal{N}\left( 0, \frac{1}{2 \ell} \right)$. Then we can show that the operator norm of $\vec{W}$ is upper-bounded by 1 with high probability. In particular we have the following, the proof for which follows directly from Theorem 2.3.8 and Proposition 2.3.10 in \citep{tao2012topics} with appropriate scaling. Define $\ell := \max\{\ell_1, \ell_2\}$. Then with probability at least $1- \Omega(\exp(-\ell^2))$ we have that $\| \vec{W} \| \leq 1$.
  %
%  Consider the following random initialization for neural networks. Let $\{\vec{W}_p\}_{p \in [\beta]_0}$ denote the set of weight matrices. Each entry in this matrix is independently initialized by a $\mathcal{N}\left( 0, \frac{1}{2\ell} \right)$ random variable. We now argue that the operator norm of each of the matrices $\{\vec{W}_p\}_{p \in [\beta]_0}$ is upper-bounded by 1 with high probability. In particular we have the following, the proof for which follows directly from Theorem 2.3.8 and Proposition 2.3.10 in \citep{tao2012topics} with appropriate scaling. Define $\ell := \max\{\ell_1, \ell_2\}$. Let $\vec{W} \in \mathbb{R}^{\ell_1 \times \ell_2}$ be a random matrix where every entry is an independent sample from $\mathcal{N}\left( 0, \frac{1}{2 \ell} \right)$. Then with probability at least $1- \Omega(\exp(-\ell^2))$ we have that $\| \vec{W} \| \leq 1$. 
  %
%  This argument can also be extended to convolutional neural nets. Consider a 2D input $\vec{X} \in \mathbb{R}^{\ell \times \ell}$ and a filter $\vec{F} \in \mathbb{R}^{k \times k}$. The convolution operation $\vec{X} \ast \vec{F} = \vec{H} \vec{x}$ where $\vec{H} \in \mathbb{R}^{(\ell-k+1)^2 \times \ell^2}$ is a \emph{Toeplitz} matrix (assuming a stride of 1 and no padding) and $\vec{x} \in \mathbb{R}^{\ell^2 \times 1}$ is the \emph{flattened} input vector \citep{gray2006toeplitz}. Define $d_{\min} := \min\{ (\ell-k+1)^2, \ell^2\}$. Consider a randomly initialized filter where every entry of the filter is a $\mathcal{N}\left( 0, \tfrac{1}{2d_{\min}} \right)$ random matrix. It then holds that with probability at least $1-\Omega(\exp(-d_{\min}^2))$, we have $\| \vec{H} \| \leq 1$. This again follows from Theorem 2.3.8 and Proposition 2.3.10 in \citep{tao2012topics} and the fact that each column in $\vec{H}$ has at most $d_{\min}$ non-zero entries each of which is an \emph{independent} gaussian random variable.
%  
%%  \soham{this result holds for fully connected networks; also a note on how the operator norm does not change much; also how it is not exactly going to be less than 1 for convnets.}
%  
%While, in general, there is no reason to believe that such a small-weights assumption would continue to hold during optimization without explicit regularizers like weight decay, some recent work has shown evidence that the weights do not move too far away during training from the random initialization point for overparameterized neural nets \citep{neyshabur2018towards, dziugaite2017computing, nagarajan2019generalization, zou2018stochastic, allen2018convergence, du2018gradient, oymak2018overparameterized}. It is worth noting though that all these results have been shown under some restrictive assumptions, such as very wide networks. \\   %, nonetheless this property seemed to also approximately hold in all our experiments (see Appendix \ref{app:opnorm_plot} for more discussion). \\
%
%%these works provide evidence that Assumption \ref{ass:small_weight} might likely be applicable through the course of optimization and near a minimizer.
%  
%

	 We now prove concentration bounds for the gradient confusion on neural nets. %We reiterate that Corollary~\ref{thm:uniformNN} analyzes the the gradient confusion property \emph{simultaneously for all weights in a ball around the minimizer.}
	 \vspace{2mm}
%	\begin{restatable}[Concentration bounds for arbitrary depth neural networks]{theorem}{NeuralNet}
	\begin{restatable}{theorem}{NeuralNet}
    	\label{thm:arbitraryNN}
    	Consider the problem of training neural nets (equation \ref{eq:NNmodel}) using either the square-loss or the logistic-loss function. Let $\eta > 0$ be a given constant. Let the weights satisfy assumption~\ref{ass:small_weight} and the non-linearities in each layer satisfy properties (P1) and (P2). For some fixed constant $c >0$, the gradient confusion bound in equation \ref{confusion} holds with probability at least 
	$$\textstyle 1- N^2 \exp\left( \frac{-c d \eta^2}{16 \zeta_0^4 (\beta+2)^4} \right).$$ 
	For both the square-loss and the logistic-loss functions,  $\zeta_0 \leq 2 \sqrt{\beta}$ (from lemma \ref{lem:lossPropNeural}). 
    	\end{restatable}
	
	Thus, theorem \ref{thm:arbitraryNN} shows that, for a given dimension $d$ and number of samples $N$, when the network depth $\beta$ decreases, the probability that the gradient confusion bound in equation \ref{confusion} holds increases, and vice versa.
	%
	Note that the convergence rate results of SGD in section \ref{sec:convergence} 
	%showing fast convergence of SGD for low gradient confusion (Theorems \ref{thm:cosine} and \ref{thm:nonconvex}) 
	assume that the gradient confusion bound holds at every point along the path of SGD. On the other hand, theorem \ref{thm:arbitraryNN} shows concentration bounds for the gradient confusion at a fixed weight $\vW$. Thus, to ensure that the above result is relevant for the convergence of SGD on overparameterized models, we now make the concentration bound in theorem \ref{thm:arbitraryNN} \emph{uniform over all weights inside a ball $\mathcal{B}_r$ of radius $r$}. \vspace{2mm}
    	
    	\begin{restatable}[Uniform concentration for all weights around the minimizer]{corollary}{NeuralNetUniform}
    		\label{thm:uniformNN}	
    	Select a point $\vec{W} = (\vec{W}_0, \vec{W}_1, \ldots, \vec{W}_\beta)$, satisfying assumption \ref{ass:small_weight}. Consider a ball $\mathcal{B}_r$ centered at $\vec{W}$ of radius $r > 0$. If the data $\{\vxi\}_{i \in [N]}$ are sampled uniformly from a unit sphere, then the gradient confusion bound in equation \ref{confusion} holds uniformly at all points $\vec{W}' \in \mathcal{B}_r$ with probability at least
    	\begin{align*}
			& \textstyle 1- N^2 \exp\left(-\frac{cd\eta^2}{64\zeta_0^4 (\beta+2)^4} \right), \hspace{19mm}\text{ if } r\le \eta/4\zeta_0^2, \\ 
&  \textstyle 1- N^2 \exp\left(-\frac{cd\eta^2}{64\zeta_0^4 (\beta+2)^4} + \frac{8d\zeta_0^2 r}{\eta}\right), \quad\quad\text{ otherwise}.
\end{align*}
    \end{restatable}
%
Thus, corollary \ref{thm:uniformNN} shows that the probability that the gradient confusion bound holds decreases with increasing depth, for all weights in a ball around the minimizer.
This explains why training very deep models is hard and typically slow with SGD \citep{bengio1994learning,glorot2010understanding}. 
Note that this is also related to the \emph{shattered gradients} phenomenon \citep{balduzzi2017shattered} that arises with depth (see appendix \ref{sec:related_work} for more discussion).
This naturally raises the question why modern deep neural networks are so efficiently trained using SGD. While careful initialization strategies prevent vanishing or exploding gradients making deeper networks trainable, these strategies still suffer from high gradient confusion for very deep networks  (as we show below in theorem \ref{thm:fixedData}).
% (see \cite{zhang2019fixup} for recent progress in this direction). 
 Thus, in section \ref{sec:experiments}, we empirically study how popular techniques like skip connections \citep{he2016deep} and batch normalization \citep{ioffe2015batch} affect gradient confusion. We find that these techniques drastically lower gradient confusion, making very deep networks significantly easier to train.
%
    Note that the above results automatically hold for convolutional nets, since a convolution operation on $\vx$ can be represented as a matrix multiplication $\vec{U}  \vec{x}$ for an appropriate Toeplitz matrix $\vec{U}$.


==> linearNN.tex <==
\subsubsection{Linear neural networks}	
	\label{sec:linear_nn}
	
	\soham{Add a note on why looking at linear neural networks is interesting: understanding the effect of depth without increasing model complexity over linear regression.}

We now study the behavior of gradient confusion for neural networks.  We begin with the simplified case of linear neural networks (i.e., with no non-linearities) with one output feature, one hidden layer.  We'll then examine the case of more general networks. 

Let $\vec{W}_0 \in \mathbb{R}^{d \times \ell_1}, \vec{W}_1 \in \mathbb{R}^{\ell_1 \times 1}$ denote the weight matrices connecting the input layer to the hidden layer, and the hidden layer to the output, respectively. Thus, the output of the neural net is given by $\vec{W}_1 \cdot  \vec{W}_0 \cdot \vec{x}$. Then we have, 
	\[
		g(\vec{x}) = \sum_{p \in [d]} \sum_{p' \in [\ell_1]} (\vec{W}_1)_{p'} (\vec{W}_0)_{p, p'} (\vec{x})_p.
	\]

Later, we consider the case of more than one hidden-layer, and use $\ell_i$ to denote the width of layer $i$ and $\beta$ to be the total number of hidden layers. Further we define $\ell := \max_{i \in [\beta]} \ell_i$. Similar to the case for linear models, we prove the following theorem.  
		
	\begin{restatable}[Bounded gradient confusion for single layer linear neural network]{thm}{singleLayer}
    	\label{thm:singleNeuralNetwork}
    	Consider a single hidden layer neural network with fixed weight vectors $\vec{W}_1 \in \mathbb{R}^{1 \times \ell_1}, \vec{W}_0 \in \mathbb{R}^{\ell_1 \times d}$ satisfying Assumption \ref{ass:small_weight}, and let $\eta >0$ be a given constant. We have that with probability at least $1-\Omega\left( n^2 \exp(-c_1 d \eta^2) \right)$, equation~\eqref{eq:mainTheorem} holds. 
    	 \end{restatable}

	Note that from Theorem~\ref{thm:singleNeuralNetwork} we have that the concentration gets sharper as the dimension of the data increases. However, it is independent of the dimension of the hidden layer. As long as $\|\vec{W}\| \leq 1$, we can train wider networks as fast as networks that are not as wide.

	\xhdr{Extension to arbitrary depth linear neural nets}
	We now extend the above analysis to an arbitrary depth linear neural network.  Interestingly, we see in this case that the gradient confusion depends critically on the network architecture -- in particular the width and depth.
	
	  In this case we have the model $g(\vec{x}) := \vec{W}_{\beta} \vec{W}_{\beta-1} \ldots \vec{W}_1 \vec{W}_0 \vec{x}$ where $\{\vec{W}_i\}_{i \in [\beta]_0}$ are weight matrices of appropriate dimensions. We let $\beta$ denote the number of layers in our hidden network, and we let $\ell$ denote the width of our network -- i.e., the maximal number of features in any layer.

	\begin{restatable}[Extension to arbitrary depth linear neural networks]{thm}{LinearNN}
    	\label{thm:arbitraryLinearNN}
    	Consider an arbitrary depth linear neural network that satisfies assumptions B1-B4 and assume the weights satisfy Assumption \ref{ass:small_weight}.
	Let $\eta >0$ be a given constant. With probability at least $1- n^2 \exp\left( \frac{-c d\eta^2}{16(\beta+1)^2 \alpha_0^4} \right)$ we have that equation~\eqref{eq:mainTheorem} holds. For both the square-loss and the logistic-loss functions, the value of $\alpha_0 \leq 2$. 
	\end{restatable}

	\begin{restatable}[Uniform concentration]{thm}{linearNNuniform}
 		\label{thm:linearNNNuniform}
	For a linear neural net that satisfies assumption A1-A5, select a point $\vec{W} = (\vec{W}_0, \vec{W}_1, \ldots, \vec{W}_\beta)$, such that for every $p \in [\beta]_0$, $\| \vec{W}_p \| \leq 1$. Consider a ball $\mathcal{B}_r$ centered at $\vec{W}$ of radius $0 < r < \eta/2\alpha_0$. If the data $\{\vxi\}_{i=1}^n$ are sampled uniformly from a unit sphere, then Equation \eqref{eq:mainTheorem} holds uniformly at all points $\vec{W} \in \mathcal{B}_r$ with probability at least
		\[
			1- n^2 \exp\left(\frac{-c d\eta^2}{64(\beta+1)^2 \alpha_0^4} \right).
		\]
		For both the square-loss and the logistic-loss functions, the value of $\alpha_0 \leq 2 \sqrt{\beta}$.
 	\end{restatable}


==> linearNNProof.tex <==
\subsection{Linear Neural Networks}
We now study the behavior of gradient confusion for linear neural networks (i.e., with no non-linearities) with one output feature.	
We start with the simplest setting of one hidden layer. Let $\vec{W}_0 \in \mathbb{R}^{\ell_1 \times d}, \vec{W}_1 \in \mathbb{R}^{1 \times \ell_1}$ denote the weight matrices connecting the input layer to the hidden layer, and the hidden layer to the output, respectively. Then we have, 
\[
	g(\vec{x}) =\vec{W}_1 \cdot \vec{W}_0 \cdot \vec{x}.
\]

Later, we consider the case of more than one hidden-layer, and use $\ell_i$ to denote the width of layer $i$ and $\beta$ to be the total number of hidden layers. Further we define $\ell := \max_{i \in [\beta]} \ell_i$. Throughout this sub-section we make the following assumption.

	Consider a $i \in [n]$. We can write $\nabla f_i (\vec{W}_1, \vec{W}_0)$ as follows.
	\begin{align*}
		\nabla_{\vec{W}_1} f_i (\vec{W}_1, \vec{W}_0) &= \alpha_i (\vec{x}_i^T \cdot \vec{W}_0^T), \\
		\nabla_{\vec{W}_0} f_i (\vec{W}_1, \vec{W}_0) &= \alpha_i (\vec{W}_1 \cdot \vec{x}_i^T).
	\end{align*}
	where $\alpha_i = f'_i(\vec{W}_1, \vec{W}_0)$.

 Thus, the expression $\langle \nabla f_i (\vec{W}_1, \vec{W}_0) , \nabla f_j (\vec{W}_1, \vec{W}_0) \rangle$ can be written as follows.
	\[
			\textstyle h(\vec{x}_i, \vec{x}_j):= \alpha_i \alpha_j \underbrace{\left( \Tr(\vec{W}_0 \cdot \vec{x}_i \cdot \vec{x}_j^T \cdot \vec{W}_0^T) + \Tr(\vec{x}_i \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \vec{x}_j^T) \right)}_{:=\kappa_{i, j}}.
	\]	
	
	

%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
			\[
				\textstyle h(\vec{x}_i, \vec{x}_j):= \alpha_i \alpha_j \underbrace{\left( \sum_{p'' \in [\ell_1]} \sum_{p \in [d]} \sum_{p' \in [d]} (\vec{W}_0)_{p, p''} (\vec{W}_0)_{p', p''} (\vec{x}_i)_p (\vec{x}_j)_{p'} + \sum_{p' \in [\ell_1]} \sum_{p \in [d]} (\vec{W}_1)^2_{p'} (\vec{x}_i)_p (\vec{x}_j)_p \right)}_{=:\kappa_{i, j}}.
			\]
		Similar to the case for linear regression, we will prove the following theorem.
\end{comment}		
	\singleLayer*
    \begin{proof}
  
    	We will prove the two properties.
    	
    \xhdr{Bounded Gradient.} As before we consider $\|\nabla_{(\vec{x}_i, \vec{x}_j)}  h(\vec{x}_i, \vec{x}_j)\|_2$. Consider $\nabla_{\vec{x}_i} h(\vec{x}_i, \vec{x}_j)$ (gradient with respect to $\vec{x}_j$ holds symmetrically). This can be written as follows.
	\[
		(\nabla_{\vec{x}_i} \alpha_i) \alpha_j \left( \Tr(\vec{W}_0 \cdot \vec{x}_i \cdot \vec{x}_j^T \cdot \vec{W}_0^T) + \Tr(\vec{x}_i \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \vec{x}_j^T) \right) + \alpha_i \alpha_j \left( \vec{W}_0^T \cdot \vec{W}_0 \cdot \vec{x}_j + \vec{x}_j \cdot \vec{W}_1 \cdot \vec{W}_1^T \right).
	\]
	From the rotation property of $\Tr(..)$, namely $\Tr(\vec{X} \cdot \vec{Y} \cdot \vec{Z}) = \Tr(\vec{Z} \cdot \vec{X} \cdot \vec{Y})$, we have that 
	\[
			\Tr(\vec{W}_0 \cdot \vec{x}_i \cdot \vec{x}_j^T \cdot \vec{W}_0^T) = \Tr(\vec{W}_0^T \cdot \vec{W}_0 \cdot \vec{x}_i \cdot \vec{x}_j^T) = \Tr(\vec{x}_j^T \cdot \vec{W}_0^T \cdot \vec{W}_0 \cdot \vec{x}_i) = \vec{x}_j^T \cdot \vec{W}_0^T \cdot \vec{W}_0 \cdot \vec{x}_i.
	\]
	Likewise, we get,
	\[
			 \Tr(\vec{x}_i \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \vec{x}_j^T) = \Tr(\vec{x}_j^T \cdot \vec{x}_i \cdot \vec{W}_1 \cdot \vec{W}_1^T) = \vec{x}_j^T \cdot \vec{x}_i \cdot \vec{W}_1 \cdot \vec{W}_1^T.
	\]
	Thus, we have,
	\[
			\|\nabla_{(\vec{x}_i, \vec{x}_j)}  h(\vec{x}_i, \vec{x}_j)\|_2 \leq 8 \alpha_0^2.
	\]

	%%%%%%%%%%%%%%%%% Old Proof %%%%%%%%%%%%%%%%%%
	\begin{comment}
    	Fix an arbitrary value $\vec{x}_i=\tilde{\vec{x}}_i$ and $\vec{x}_j=\tilde{\vec{x}}_j$. Consider an arbitrary coordinate corresponding to the variable $(\vec{x}_i)_p$ (by symmetry a corresponding argument holds for $(\vec{x}_j)_p$) in the vector $\vec{\nabla h(x, y)}$. The term evaluates to the following.
			
			\begin{align*}
    			&\textstyle \alpha_i \alpha_j \left( \sum_{p'' \in [\ell_1]} \sum_{p' \in [d]} (\vec{W}_0)_{p, p''}(\vec{W}_0)_{p', p''} (\vec{x}_j)_{p'} +\sum_{p' \in [\ell_1]} (\vec{W}_1)^2_{p'}(\vec{x}_j)_p \right) \\
    			& \textstyle + \alpha_j \kappa_{i, j} \left( \sum_{p' \in [\ell_1]} (\vec{W}_1)_{p'} (\vec{W}_0)_{p, p'} - (\tilde{\vec{W}})_p \right).
			\end{align*}
			
			By the assumption that both $\cC(\vec{x})$ and $g(\vec{x})$ lie between $[-1, 1]$, we have that $-2 \leq \alpha_i \leq 2$ for all $i \in [n]$. From Assumption \ref{ass:small_weight} and the sampling procedure of $\vec{x}_i$'s we have the following.
				\begin{equation}
					\label{eq:firstLayerObs_supp}
						\sum_{p \in [d]} (\vec{W}_0)_{p, p''} (\vec{x}_i)_p \leq \frac{1}{\ell_1} \sum_{p \in [d]} (\vec{x}_i)_p \leq \frac{1}{\ell_1}.
				\end{equation}
			Hence, combining this with Assumption \ref{ass:small_weight}, the first term in the sum above can be upper-bounded by $8/\ell_1$. Note that for every pair $i, j \in [n]$ we have that $-1 \leq \sum_{p \in [d]} (\vec{x}_i)_p (\vec{x}_j)_p \leq 1$ since this quantity represents the cosine of the angle between two vectors. Again using the observation in Equation~\eqref{eq:firstLayerObs_supp} and Assumption \ref{ass:small_weight}, we have that $\kappa_{i, j} \leq 2/\ell_1$. Hence, the second term in the summand above can be upper-bounded by $8/\ell_1$ and hence $||\vec{\nabla(h(x_i, x_j))}||_{\infty} \leq 16/\ell_1$. In other words, we have that $\rho$ is $O(1/\ell_1)$.
		\end{comment}

			\xhdr{Non-negative Expectation.}
		As in the case of linear regression, we can write,
		\begin{align*}
		\mathbb{E}_{\vxi,\vxj}[h(\vec{x}_i, \vec{x}_j)] =& \mathbb{E}_{\vxi,\vxj}[\langle \nabla f_i (\vec{W}_1, \vec{W}_0) , \nabla f_j (\vec{W}_1, \vec{W}_0) \rangle] \\
		&= \langle \mathbb{E}_{\vxi}[ \nabla f_i (\vec{W}_1, \vec{W}_0)] , \mathbb{E}_{\vxj}[\nabla f_j (\vec{W}_1, \vec{W}_0) ] \rangle \\
		&= \|\mathbb{E}_{\vxi}[ \nabla f_i (\vec{W}_1, \vec{W}_0)]\|^2\ge 0.
		\end{align*}
We have used the fact that $\nabla f_i (\vec{W}_1, \vec{W}_0)$ and $ \nabla f_j (\vec{W}_1, \vec{W}_0)$ are identically distributed and independent.
		
		%	To compute bounds on $\mathbb{E}[h(\vec{x}_i, \vec{x}_j)]$, we use the law of total expection. We have 
		%	$$\mathbb{E}[\alpha_i \alpha_j \langle \vec{x}_i, \vec{x}_j \rangle] = \mathbb{E}[\langle \alpha_i\vec{x}_i,  \alpha_j \vec{x}_j \rangle] = 
		%	 \langle \mathbb{E}[\alpha_i\vec{x}_i],  \mathbb{E}[\alpha_j \vec{x}_j ]\rangle  = \|\mathbb{E}[\alpha_i\vec{x}_i]\|^2\ge 0.$$
		%	 Note we have used the fact that $\alpha_i\vec x_i$ and $\alpha_j \vec x_j$ are independent and identically distributed.
			
			
		%	Note that $\alpha_i, \alpha_j \geq -\alpha_0$. Therefore we have $\mathbb{E}[h(\vec{x}_i, \vec{x}_j)] \geq -\alpha_0^2 \mathbb{E}[\kappa_{i, j}]$. By using Linearity of Expectation, mutual independence of $\vec{x}_i$ and $\vec{x}_j$ and the fact that normalized Gaussian random variables have mean $0$ at every co-ordinate, we have that $\mathbb{E}[\kappa_{i, j}] = 0$. Therefore we have $\mathbb{E}[h(\vec{x}_i, \vec{x}_j)] \geq 0$.
			
			Armed with the bounded gradient and non-negative expectation properties, the rest of the proof follows as in the proof of Theorem \ref{thm:linearRegression}. 
\qedhere
    \end{proof}




\subsection{Extension to arbitrary length linear networks}

	We now extend the above analysis to an arbitrary depth linear neural network. We have 
	\[
		g(\vec{x}) := \vec{W}_{\beta} \cdot \vec{W}_{\beta-1} \cdot \ldots \vec{W}_0 \cdot \vec{x}.
	\]	
	 Let $h(\vec{x}_i, \vec{x}_j) := \langle \nabla f_i (\vec{W}_{\beta}, \ldots, \vec{W}_0), \nabla f_j(\vec{W}_{\beta}, \ldots, \vec{W}_0) \rangle$. 

	\LinearNN*
	
	\begin{proof}
		We now show the two properties on $h(. , .)$ as we did for the simpler cases.
		
		\xhdr{Bounded gradient.}
		For every $i \in [n]$ define $\alpha_i := f'(\vec{W}_\beta, \vec{W}_{\beta-1}, \ldots, \vec{W}_0)$. Then we have the following. 
		\begin{align*}
			\nabla_{\vec{W}_0} f_i (\vec{W}_{\beta}, \ldots, \vec{W}_0) &= \alpha_i (\vec{W}_1^T \cdot \vec{W}_2^T \cdot \ldots \cdot \vec{W}_\beta^T \cdot \vec{x}_i^T), \\
			 \nabla_{\vec{W}_p} f_i (\vec{W}_{\beta}, \ldots, \vec{W}_0) &= \alpha_i (\vec{W}_{p+1}^T \cdot \ldots \cdot \vec{W}_\beta^T \cdot \vec{x}_i^T \cdot \vec{W}_0^T \cdot \ldots \cdot \vec{W}_{p-1}^T) & \forall p \in [\beta].
		\end{align*}

		For notational convenience we define the following quantities.
		\begin{align*}
			A_0(\vec{x}_i, \vec{x}_j) &:=	\vec{x}_i \cdot \vec{W}_\beta \cdot \ldots \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \ldots \vec{W}_{\beta}^T \cdot \vec{x}_j^T. \\
			A_p(\vec{x}_i, \vec{x}_j) &:= \vec{W}_{p-1} \cdot \ldots \vec{W}_0 \cdot \vec{x}_i \cdot \vec{W}_{\beta} \cdot \ldots \cdot \vec{W}_{p+1} \cdot \vec{W}_{p+1}^T \cdot \ldots \cdot \vec{W}_{\beta}^T \cdot \vec{x}_j^T \cdot \vec{W}_0^T \cdot \ldots \cdot \vec{W}_{p-1}^T.
		\end{align*}


		Thus, $h(\vec{x}_i, \vec{x}_j)$ can be written as 
		\[
			\alpha_i \alpha_j \left( \sum_{p \in [\beta]_0} \Tr[ A_p(\vec{x}_i, \vec{x}_j) ]\right).
		\]
		We will now bound $\|\nabla_{(\vec{x}_i, \vec{x}_j)} h(\vec{x}_i, \vec{x}_j) \|_2$. Consider 
		$\nabla_{\vec{x}_i} h(\vec{x}_i, \vec{x}_j)$. This can be written as follows.
		\begin{multline}
			\label{eq:linNNMain}
			(\nabla_{\vec{x}_i} \alpha_i) \alpha _j \left( \sum_{p \in [\beta]_0} \Tr[ A_p(\vec{x}_i, \vec{x}_j) ]\right) +\\
			 \alpha_i \alpha_j (\vec{x}_j \cdot \vec{W}_\beta \cdot \ldots \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \ldots \cdot + \vec{W}_\beta^T) + \\
			 \alpha_i \alpha_j \sum_{p \in [\beta]} \vec{W}_0^T \cdot \ldots \cdot \vec{W}_{p-1}^T \cdot
			 \vec{W}_{p-1} \cdot \ldots \cdot \vec{W}_0 \cdot \vec{x}_j \cdot \vec{W}_{\beta} \cdot \ldots \vec{W}_{p+1} \cdot \vec{W}_{p+1}^T \cdot \ldots \cdot \vec{W}_\beta^T.
		\end{multline}
		Consider $\Tr[A_0(\vec{x}_i, \vec{x}_j) ]$. Using the rotation property of $\Tr[..]$ we obtain,
		\[
				\Tr[A_0(\vec{x}_i, \vec{x}_j) ] = \Tr[ \vec{x}_j^T \cdot \vec{x}_i \cdot \vec{W}_\beta \cdot \ldots \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \ldots \vec{W}_{\beta}^T] = \vec{x}_j^T \cdot \vec{x}_i \cdot \vec{W}_\beta \cdot \ldots \cdot \vec{W}_1 \cdot \vec{W}_1^T \cdot \ldots \vec{W}_{\beta}^T.
		\]
		Likewise using the rotation property of $\Tr[..]$, for every $p \in [\beta]$ we obtain,
		\begin{align*}
				\Tr[A_p(\vec{x}_i, \vec{x}_j)] &= \Tr[\vec{x}_j^T \cdot \vec{W}_0^T \cdot \ldots \cdot \vec{W}_{p-1}^T \cdot \vec{W}_{p-1} \cdot \ldots \cdot \vec{W}_0 \cdot \vec{x}_i \cdot \vec{W}_{\beta} \cdot \ldots \cdot \vec{W}_{p+1} \cdot \vec{W}_{p+1}^T \cdot \ldots \cdot \vec{W}_{\beta}^T]\\
				&=\vec{x}_j^T \cdot \vec{W}_0^T \cdot \ldots \cdot \vec{W}_{p-1}^T \cdot \vec{W}_0 \cdot \ldots \cdot \vec{W}_{p-1} \cdot \vec{x}_i \cdot \vec{W}_{\beta} \cdot \ldots \cdot \vec{W}_{p+1} \cdot \vec{W}_{p+1}^T \cdot \ldots \cdot \vec{W}_{\beta}^T.
		\end{align*}
		Thus, using Assumption~\ref{ass:small_weight} and Equation~\eqref{eq:linNNMain} we obtain $\|\nabla_{(\vec{x}_i, \vec{x}_j)} h(\vec{x}_i, \vec{x}_j)\|_2 \leq 4 (\beta+1) \alpha_0^2$.
			
	\xhdr{Non-negative expectation.} This follows from the same argument made in the case of a single hidden layer net.
    	%As before, using the fact that $\alpha_i \geq -\alpha_0$ and $\alpha_j \geq -\alpha_0$ and normalized gaussian random variable has mean $0$, we have that $\mathbb{E}[h(\vec{x}_i, \vec{x}_j)] \geq 0$. 
\end{proof}

	
	%%%%%%%%%%%%%%%%%%% Old Proof %%%%%%%%%%%%%%%%%%%
	\begin{comment}
	\begin{proof}
		This statement can be equivalently written as follows. Note that for constants $c', c'' > 0$, we want $c' n^2 \exp( \frac{-c \ell^2 d \eta^2}{\beta^2} ) \leq c'' \frac{1}{\textsf{poly}(d)},$, since we we assume that $d$ is the asymptotic parameter and hence this makes the concentration explicit. Rearranging and solving for $d$, we get the condition that $d \geq \Omega( (\beta/\ell)^2 \log n)$. 
		
		We now show the two properties on $h(. , .)$ as we did for the simpler cases.
		
		\xhdr{Bounded gradient.}
		We will first compute $\nabla f_i (\vec{W}_{\beta}, \ldots, \vec{W}_0)$. Note that the gradient can be visualized as follows. The first $\ell_{\beta}$ entries correspond to the entries in $\frac{\partial f_i}{\partial \vec{W}_{\beta}}$. The next $\ell_{\beta} * \ell_{\beta-1}$ entries correspond to $\frac{\partial f_i}{\partial \vec{W}_{\beta-1}}$ and so on.
		
		These entries can be computed as follows. 
		\begin{equation*}
			\left( \frac{\partial f_i}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}} = \alpha_i \left( \sum_{p_{\beta-1} \in [\ell_{\beta-1}]} \ldots \sum_{p_1 \in [\ell_1]} \sum_{p \in [d]} (\vec{W}_{\beta-1})_{p_{\beta}, p_{\beta-1}} \ldots (\vec{W}_0)_{p_{1}, p} (\vec{x}_i)_p \right) .
		\end{equation*}
		
		\begin{multline*}
			\left( \frac{\partial f_i}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}} = \alpha_i \Bigg( \sum_{p_{\beta} \in [\ell_{\beta}]} \ldots \sum_{p_{\beta'+2} \in [\ell_{\beta' + 2}]} \sum_{p_{\beta'-1} \in [\ell_{\beta' -1}]} \ldots \sum_{p_1 \in [\ell_1]} \sum_{p \in [d]} \\
			(\vec{W}_{\beta})_{p_{\beta}} (\vec{W}_{\beta-1})_{p_{\beta}, p_{\beta-1}} \ldots (\vec{W}_{\beta'+1})_{p_{\beta'+2}, p_{\beta'+1}} (\vec{W}_{\beta'-1})_{p_{\beta'}, p_{\beta'-1}} \ldots  (\vec{W}_0)_{p_{1}, p} (\vec{x}_i)_p \Bigg) \\ \qquad \forall \beta' \in \{1, 2, \ldots, \beta-1\}.
		\end{multline*}

		\begin{equation*}
			\left( \frac{\partial f_i}{\partial \vec{W}_{0}} \right)_{p_1, p} = \alpha_i \left( \sum_{p_{\beta} \in [\ell_{\beta}]} \ldots \sum_{p_2 \in [\ell_2]}  (\vec{W}_{\beta})_{p_{\beta}} \ldots (\vec{W}_1)_{p_2, p_1} (\vec{x}_i)_p \right). 
		\end{equation*}


		Hence $h(\vec{x}_i, \vec{x}_j)$ can be written as follows.
		\begin{multline*}
			h(\vec{x}_i, \vec{x}_j) = \sum_{p_{\beta} \in [\ell_\beta]} \underbrace{\left( \frac{\partial f_j}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}} \left( \frac{\partial f_i}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}}}_{=: \psi_\beta}  + \sum_{\beta' \in [\beta-1]} \sum_{p_{\beta' + 1} \in [\ell_{\beta' +1}]} \sum_{p_{\beta'} \in [\ell_{\beta'}]} \underbrace{\left( \frac{\partial f_j}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}} \left( \frac{\partial f_i}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}}}_{=:\psi_{\beta'}}\\
			+ \sum_{p_1 \in [\ell_1]}\sum_{p \in [d]} \underbrace{\left( \frac{\partial f_j}{\partial \vec{W}_{0}} \right)_{p_1, p} \left( \frac{\partial f_i}{\partial \vec{W}_{0}} \right)_{p_1, p}}_{=:\psi_0}.
		\end{multline*}

	The following claim can be obtained as a consequence of Assumption \ref{ass:small_weight}.
	
	\begin{lemma}
		\label{lem:linNNA1_supp}
		For simplicity of notation in this Lemma, denote $\ell_0 := d$. Let $\vec{W}_0 \in [-1/\ell, 1/\ell]^{\ell_1 \times \ell_0}, \vec{W}_1 \in [-1/\ell, 1/\ell]^{\ell_2 \times \ell_1}, \ldots, \vec{W}_\beta \in [-1/\ell, 1/\ell]^{1 \times \ell_\beta}$ be weight matrices satisfying Assumption \ref{ass:small_weight}. Then for any given $\beta' \in \{1, \ldots, \beta\}$ and $p_{\beta'} \in \{0, 1, 2, \ldots, \ell_{\beta'}\}$, we have that any product consisting of a sequence of matrices $\vec{W}_\beta \cdot \vec{W}_{\beta-1} \cdot \ldots \cdot (\vec{W}_{\beta'})_{p_{\beta'}}$ lies in the interval $[-1/\ell, 1/\ell]$.
	\end{lemma}
	
	\begin{proof}
		For notational convenience, denote the column vector $(\vec{W}_{\beta'})_{p_{\beta'}}$ as $\overline{\vec{W}}_0$. Define $\nu := \beta-\beta'$. We also rewrite the chain $\vec{W}_\beta \cdot \vec{W}_{\beta-1} \cdot \ldots (\vec{W}_{\beta'})_{p_{\beta'}}$ as $\overline{\vec{W}}_\nu \cdot \overline{\vec{W}}_{\nu-1} \cdot \ldots \cdot \overline{\vec{W}}_0$. We will now prove that the value of this matrix-vector product lies in the interval $[-1/\ell, 1/\ell]$. By induction on $\nu$, we will prove that the product $\overline{\vec{v}}_\nu:=\overline{\vec{W}}_{\nu-1} \cdot \ldots \cdot \overline{\vec{W}}_0$ will always yield a column vector where every entry lies in the interval $[-1/\ell, 1/\ell]$. Given the proof of this inductive hypothesis, note that we have the following inner-product $\langle \overline{\vec{W}}_\nu, \vec{v}_\nu \rangle$ where every entry in both these vectors lies in the interval $[-1/\ell, 1/\ell]$. Since the dot-product is a sum over at most $\ell$ terms with each term in the sum bounded in the interval $[-1/\ell^2, 1/\ell^2]$, we have that the dot-product lies in the interval $[-1/\ell, 1/\ell]$.
		
		We will now prove the inductive statement. The base-case is when $\nu=1$. In this case we have a single vector $\overline{\vec{W}}_0$. By assumption we have that each entry in this vector lies in the interval $[-1/\ell, 1/\ell]$ and therefore the hypothesis is true.
		Consider the case when $\nu > 1$. Consider the chain $\overline{\vec{v}}_\nu:=\overline{\vec{W}}_{\nu-1} \cdot \overline{\vec{W}}_{\nu-2} \cdot \ldots \cdot \overline{\vec{W}}_0$. From the inductive hypothesis, we have that $\overline{\vec{v}}_{\nu-1}:=\overline{\vec{W}}_{\nu-2} \cdot \ldots \cdot \overline{\vec{W}}_0$ gives a column vector where every entry is in the interval $[-1/\ell, 1/\ell]$. Consider the $i$-th entry in the column vector $\overline{\vec{v}}_\nu$. This is obtained by the inner product of the $i$-th row of matrix $\overline{\vec{W}}_{\nu-1}$ and the column vector $\overline{\vec{v}}_{\nu-1}$. Since this is a sum of at most $\ell$ term with each term in the interval $[-1/\ell^2, 1/\ell^2]$, we have that this $i$-th entry lies in the interval $[-1/\ell, 1/\ell]$.
	\end{proof}
	In the analysis for general neural networks, we use the following corollary.
	\begin{corollary}
		\label{cor:chainMatrices}
			Let $\vec{W}_0 \in [-1/\ell, 1/\ell]^{\ell_1 \times \ell_0}, \vec{W}_1 \in [-1/\ell, 1/\ell]^{\ell_2 \times \ell_1}, \ldots, \vec{W}_\beta \in [-1/\ell, 1/\ell]^{1 \times \ell_\beta}$ be weight matrices satisfying Assumption \ref{ass:small_weight}. Then for any given $\beta \leq \beta' \leq 1$, we have that any product consisting of a sequence of matrices $\vec{W}_{\beta'} \cdot \vec{W}_{\beta'-1} \cdot \ldots \vec{W}_0 \cdot \vec{x}$ lies in the interval $[-1/\ell, 1/\ell]$, where $\vec{x}$ is a normalized Gaussian.
	\end{corollary}
	\begin{proof}
		The proof of this follows directly by combining Equation~\ref{eq:firstLayerObs_supp} and the above Lemma \ref{lem:linNNA1_supp}.
	\end{proof}
	
	
	
	We now use Lemma \ref{lem:linNNA1_supp} to bound the value of $||\vec{\nabla h}||_{\infty}$. Consider any fixed $\vec{x}_i = \tilde{\vec{x}}_i$ and $\vec{x}_j = \tilde{\vec{x}}_j$. Consider the entry corresponding to $(\vec{x}_i)_p$. We have that each entry in $\nabla f_i (\vec{W}_{\beta}, \ldots, \vec{W}_0)$ is at most $3/\ell$. This is because of the fact that $\alpha_i \leq 2$ and the terms involving the product-chain of weight matrices is at most $1/\ell$.  
		In particular it is at most $1/\ell$ in case of $\left( \frac{\partial f_i}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}}$ and $\left( \frac{\partial f_i}{\partial \vec{W}_{0}} \right)_{p_1, p}$ (from Corollary \ref{cor:chainMatrices}) and $1/\ell^2$ in case of $\left( \frac{\partial f_i}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}}$ (using both Corollary \ref{cor:chainMatrices} and Lemma \ref{lem:linNNA1_supp}).
	
		Notice that in the expression for $h(.,.)$, the $(\vec{x}_i)_p$ terms appear in $\alpha_i$ and $\frac{\partial f_i}{\vec{W}_{\beta'}}$, for $\beta' \in \{0, 1, \ldots, \beta\}$, terms only.
	
		The co-ordinate corresponding to $(\vec{x}_i)_p$ in $\nabla h$ can be written as the following sum.
		\begin{equation}
			\label{eqn:derivateX}
				\sum_{p_\beta \in [\ell_\beta]} \frac{\partial \psi_{\beta}}{\partial (\vec{x}_i)_p} + \sum_{\beta' \in [\beta-1]} \sum_{p_{\beta' + 1} \in [\ell_{\beta' +1}]} \sum_{p_{\beta'} \in [\ell_{\beta'}]} \frac{\partial \psi_{\beta'}}{\partial (\vec{x}_i)_p} + \sum_{p_1 \in [\ell_1]}\sum_{p \in [d]} \frac{\partial \psi_{0}}{\partial (\vec{x}_i)_p}
		\end{equation}
		
		We will now compute each of these partial derivatives. We will frequently come across the following term in these expressions, namely, $\frac{\partial \alpha_i}{\partial (\vec{x}_i)_p}$. This evaluates to $\left( \vec{W}_\beta \cdot \vec{W}_{\beta-1} \cdot \ldots \cdot (\vec{W}_0)_p - \underbrace{\frac{\partial \mathcal{C}(\vec{x})}{\partial (\vec{x}_i)_p}}_{=(\tilde{\vec{W}})_p} \right)$. Using the fact that $|(\tilde{\vec{W}})_p| \leq 1$, we can upper bound this by $2$. We denote this term by $\alpha_i'$ in the following expressions.
		
		\begin{multline*}
			\frac{\partial \psi_{\beta}}{\partial (\vec{x}_i)_p} = \left( \frac{\partial f_j}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}} \left[ \left( \sum_{p_{\beta-1} \in [\ell_{\beta-1}]} \ldots \sum_{p_1 \in [\ell_1]} \sum_{p \in [d]} (\vec{W}_{\beta-1})_{p_{\beta}, p_{\beta-1}} \ldots (\vec{W}_0)_{p_{1}, p} (\vec{x}_i)_p \right) \alpha_i' \right. \\ \left.  + \alpha_i \left( \sum_{p_{\beta-1} \in [\ell_{\beta-1}]} \ldots \sum_{p_1 \in [\ell_1]} (\vec{W}_{\beta-1})_{p_{\beta}, p_{\beta-1}} \ldots (\vec{W}_0)_{p_{1}, p} \right) \right]
		\end{multline*}
	
		Using Lemma~\ref{lem:linNNA1_supp}, Corollary~\ref{cor:chainMatrices}, $-2 \leq \alpha_i \leq 2$, $\left( \frac{\partial f_j}{\partial \vec{W}_{\beta}} \right)_{p_{\beta}} \leq \frac{3}{\ell}$ and $\alpha_i' \leq 2$, we have that $\frac{\partial \psi_{\beta}}{\partial (\vec{x}_i)_p} \leq \frac{12}{\ell^2}$
	
	
	Likewise, we can write the expressions for the other two terms. Here $\left(...\right)$ denotes the summation involving the weights in $\left( \frac{\partial f_i}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}}$.
	
		\begin{multline*}
			\frac{\partial \psi_{\beta'}}{\partial (\vec{x}_i)_p} = \left( \frac{\partial f_j}{\partial \vec{W}_{\beta'}} \right)_{p_{\beta'+1}, p_{\beta'}} \left[ \left( ... \right) \alpha_i'  + \alpha_i \Bigg( \sum_{p_{\beta} \in [\ell_{\beta}]} \ldots \sum_{p_{\beta'+2} \in [\ell_{\beta' + 2}]} \sum_{p_{\beta'-1} \in [\ell_{\beta' -1}]} \ldots \sum_{p_1 \in [\ell_1]} \right. \\ \left. 
			(\vec{W}_{\beta})_{p_{\beta}} (\vec{W}_{\beta-1})_{p_{\beta}, p_{\beta-1}} \ldots (\vec{W}_{\beta'+1})_{p_{\beta'+2}, p_{\beta'+1}} (\vec{W}_{\beta'-1})_{p_{\beta'}, p_{\beta'-1}} \ldots  (\vec{W}_0)_{p_{1}, p} \Bigg) \right]
		\end{multline*}
	
	
	Using the argument as before this can be upper-bounded as $\frac{8}{\ell^4}$. 
	
	Finally, we have the following for the last term. As before, $\left( ... \right)$ denotes the summation involving the weight-matrices in $\left( \frac{\partial f_i}{\partial \vec{W}_{0}} \right)_{p_1, p}$.
	
	\begin{multline*}
			\frac{\partial \psi_{0}}{\partial (\vec{x}_i)_p} = \left( \frac{\partial f_j}{\partial \vec{W}_{0}} \right)_{p_1, p} \left[ \left( ... \right) \alpha_i'  + \alpha_i \left( \sum_{p_{\beta} \in [\ell_{\beta}]} \ldots \sum_{p_2 \in [\ell_2]}  (\vec{W}_{\beta})_{p_{\beta}} \ldots (\vec{W}_1)_{p_2, p_1} \right)\right]
		\end{multline*}
		
		This upper-bounds to $\frac{12}{\ell^2}$.
		
		Substituting 	the upper-bounds back in Equation~\eqref{eqn:derivateX}, we have that $\rho$ is $O(\beta/\ell)$ \footnote{Note that this bound is loose. With further assumptions on relationship between $\beta$ and $\ell$ one can tighten the bound. We do not do so, to keep the presentation clean; it doesn't change the main message.}.
	
	\xhdr{Non-negative expectation.}
    	As before, using the fact that $\alpha_i \geq -2$ and $\alpha_j \geq -2$ and normalized gaussian random variable has mean $0$, we have that $\mathbb{E}[h(\vec{x}_i, \vec{x}_j)] \geq 0$. 
\end{proof}
\end{comment}

	\linearNNuniform*
	\begin{proof}
		The proof of this (almost) follows from Theorem~\ref{thm:linearuniform}. We compute an upper-bound on the quantity $\| \nabla_{\vec{W}} \alpha_i \|$. Then using the same arguments as in the proof of Theorem~\ref{thm:linearuniform} and combining with Theorem~\ref{thm:arbitraryLinearNN} we obtain the result.
		
		Consider $\| \nabla_{\vec{W}} \alpha_i \|_2$. Consider $\nabla_{\vec{W}_p} \alpha_i$ for some $p \in [\beta]_0$. We will show that $\| \nabla_{\vec{W}_p} \alpha_i \|_2 \leq 2$. Then it immediately follows that $\| \nabla_{\vec{W}} \alpha_i \|_2 \leq 2 \sqrt{\beta}$ .
		
		Consider the squared loss function. We then have the following.
		\begin{align*}
			\| \nabla_{\vec{W}_p} \alpha_i \| &= \| \nabla_{\vec{W}_p} f'(\vec{W}_{\beta}, \ldots, \vec{W}_0) \| \\
			&= \| \nabla_{\vec{W}_p} g_{\vec{W}}(\vec{x}_i) - \cC(\vec{x}_i) \| \\
			& \leq \| \nabla_{\vec{W}_p} g_{\vec{W}}(\vec{x}_i) \| + 1.	
		\end{align*}
		
		Likewise, consider the logistic-loss function. We then have the following.
		\begin{align*}
			\| \nabla_{\vec{W}_p} \alpha_i \| & \leq \norm{\frac{\cC(\vec{x}_i)^2}{(1+\exp(\cC(\vec{x}_i) g_{\vec{W}}(\vec{x}_i)))^2} \exp(\cC(\vec{x}_i) g_{\vec{W}}(\vec{x}_i))} \| \nabla_{\vec{W}_p} g_{\vec{W}}(\vec{x}_i) \| \\
			& \leq \nabla_{\vec{W}_p} g_{\vec{W}}(\vec{x}_i) \| 	
		\end{align*}
		
		Since $\|\nabla_{\vec{W}_p} g_{\vec{W}}(\vec{x}_i) \| \leq 1$, we have that $\| \nabla_{\vec{W}_p} \alpha_i \| \leq 2$ in both the cases.
	\end{proof}


==> linearRegression.tex <==
%!TEX root = main.tex
\subsection{A simple case: linear models}\label{linearmodel}
We begin by examining gradient confusion in the case of fitting a simple linear model to data. In this case, the function $g_{\vec{w}}$ can be written as follows.
  \begin{equation}
  	\label{eq:lineModel}
  	 g_{\vec w}(\vec{x}) =  \vec{w}^\top \vec x.	
  \end{equation}
  %
	As stated earlier, we consider two loss functions, namely the square loss for regression and the logistic loss for classification. Both these functions have the following useful properties.\\
\begin{restatable}{lem}{lossProp}
\label{lem:lossPropLinear}
		Consider the set of loss-functions $\{f_i(\vec{w})\}_{i \in [N]}$ where all $f_i$ are either the square-loss function or the logistic-loss function. Consider a linear model with weights $\vec{w}$ satisfying $\| \vec{w} \| \leq 1$. Consider the gradient $\nabla_{\vec{w}} f_i(\vec{w})$ of each function $f_i$. Note that we can write $\nabla_{\vec{w}} f_i(\vec{w}) = \zeta_{\vec{x}_i}(\vec{w}) \nabla_{\vec{w}}g_{\vec{w}}(\vec{x}_i)$, where we define $\zeta_{\vec{x}_i}(\vec{w}) = \partial f_i(\vec{w}) / \partial g_{\vec{w}}$. Then we have the following properties.
		\begin{enumerate}
			\item When $\| \vec{x} \| \leq 1$ we have $\| \nabla_{\vec{w}}g_{\vec{w}}(\vec{x}_i) \| \leq 1$.
			\item There exists a constant $\zeta_0 > 0$ such that $|\zeta_{\vec{x}_i}(\vec{w}) | \leq \zeta_0 \,$, $\|\nabla_{\vec{x}_i} \zeta_{\vec{x}_i}(\vec{w}) \|_2 \leq \zeta_0 \,$, $\|\nabla_{\vw} \zeta_{\vec{x}_i}(\vec{w})\|_2 \leq \zeta_0$.
		\end{enumerate}
		When $g_{\vec{w}}$ is a linear model, as defined in eq.~\ref{eq:lineModel}, we have that $\zeta_0 \leq 2$. 
	\end{restatable}
\begin{proof} See Appendix \ref{appsec:helperlemma} for the proof. \end{proof}

	Define the function $h_\vw(\vec{x}_i, \vec{x}_j) := \langle \nabla_{\vec{w}} f_i, \nabla_{\vec{w}} f_j \rangle$. The following theorem shows that, for randomly sampled data, the gradient confusion bound 
%	eq.~\eqref{confusion} 
	holds with high probability.  \\
 \begin{restatable}[Concentration for linear models]{thm}{LinearRegression}
    	\label{thm:linearRegression}
    	Consider the problem of fitting linear models (eq.~\ref{eq:lineModel}) to data using either the square-loss or the logistic-loss function. Let $\vec{w}$ be an arbitrary weight vector such that $\|\vec{w}\|_2 \leq 1$ and let $\eta >0$ be a given constant. The gradient confusion bound (eq.~\ref{confusion}) holds at $\vec{w}$ with probability at least $1-N^2 \exp\left(-\frac{cd\eta^2}{16\zeta_0^4}\right)$ for some absolute constant $c>0$. For both the square-loss and the logistic-loss functions, the value of $\zeta_0 \leq 2$.
  \end{restatable}
  \begin{proof} See Appendix \ref{appsec:linregconc} for the proof.\end{proof}	
This theorem can be interpreted as follows. As long as the dimension of the input (and thus the number of parameters in the problem) is large enough, the gradient confusion for a given weight vector is low, with high-probability. Thus, gradient confusion is lower as the linear model becomes more overparameterized, an effect that shows up in the simulation in Figure \ref{fig:linreg_simulation}.

Note that the results in Section \ref{sec:convergence} showing fast convergence of SGD for low gradient confusion (Theorems \ref{thm:cosine} and \ref{thm:nonconvex}) assume that the gradient confusion bound holds at every point along the path of SGD. On the other hand, Theorem \ref{thm:linearRegression} above shows that gradient confusion is low with high probability for overparameterized models, at a fixed weight $\vw$. Thus, to ensure that the above result is relevant for the convergence of SGD on overparameterized linear models, we now make the concentration bound in Theorem \ref{thm:linearRegression} \emph{uniform} over all weights inside a ball $\mathcal{B}_r$ of radius $r$. \\

%\begin{comment}
%\begin{figure}
%    \centering
%     \includegraphics[width=.6\linewidth]{n_100}\\
%      \caption{Simulation proof for Theorem~\ref{thm:linearRegression}.  As the dimensionality of a random linear regression problem increases, the probability of violating the gradient confusion condition $\eta>0.1$ vanishes. \soham{Change y-axis label to $Pr[min_{i, j}  \la f'_i,  f'_j\ra > 0.1]$} \tom{KILL THIS FIGURE to save space!}} 
%       \label{fig:linearRegression}
%\end{figure}  
%\end{comment}	
	
\begin{restatable}[Uniform concentration]{thm}{linearuniform}
 \label{thm:linearuniform}
Consider the problem of fitting linear models (eq.~\ref{eq:lineModel}) to data using either the square-loss or the logistic-loss function. Select a point $\vw_0$ such that $\|\vec{w}\|_2 \leq 1$, and consider a ball $\mathcal{B}_r$ centered at $\vw_0$ of radius $r>0.$ If the data $\{\vxi\}_{i \in [N]}$ are sampled uniformly from a unit sphere, then the gradient confusion bound (eq.~\ref{confusion}) holds uniformly at all points $\vw \in \mathcal{B}_r$ with probability at least
\begin{align*}
&1- N^2 \exp\left(-\frac{cd\eta^2}{64\zeta_0^4} \right), \hspace{19mm} \text{ if } r\le \eta/4\zeta_0^2, \\ 
&1- N^2 \exp\left(-\frac{cd\eta^2}{64\zeta_0^4} + \frac{8d\zeta_0^2 r}{\eta}\right), \quad\text{ otherwise}.
\end{align*}
 \end{restatable}
  \begin{proof} See Appendix \ref{appsec:linregconcunif} for the proof.\end{proof}	
Thus, as long as the radius $r$ is not too large, we see that the gradient confusion bound holds uniformly with high probability for all points within the ball $\mathcal{B}_r$.
%\begin{comment}
%	\subsubsection{Technical approach \& proof sketch} \tom{REMOVE this proof sketch for ICML.  It describes standard methods and makes our proofs sound easy.  It also takes up space}
%		To prove that any bound on the gradient confusion $\eta>0$ is attained for sufficiently large $d,$ we examine the values of the function $h(\vec{x}_i, \vec{x}_j) := \langle \nabla f_i, \nabla f_j \rangle$ when $\vec{x}_i$ and $\vec{x}_j$ are selected at random from the unit sphere.  Our goal will be to show that this function has positive expected value, and that $h$ concentrates around its expected value for large $d,$ thus making it extremely unlikely that a large negative value of $h$ is observed.  Once we have shown that $h(\vec{x}_i, \vec{x}_j)< -\eta$ with extremely low probability for a random pair of points $(\vec{x}_i, \vec{x}_j),$ we can use a union bound to show that this occurs with low probability for all pairwise comparisons between data points. 
%
%For a given constant $\eta > 0$, our goal is to find a sharp bound $\tau(n, d, \eta)$ such that for a fixed $i,j$
%       %
%       \begin{equation}
%          \label{eq:conc_func}
%         \textstyle \Pr[ h(\vec{x}_i, \vec{x}_j) \leq -\eta] \leq \tau(n, d, \eta).
%       \end{equation}
%       %
%       By using the union bound and the fact that $h(\vec{x}_i, \vec{x}_j)$ is identically distributed for all $i,j \in [n]$, we have that 
%       \begin{equation}
%          \label{eq:conc_func2}
%       		 \textstyle \Pr[\exists  i \neq j, h(\vec{x}_i, \vec{x}_j)  \leq  -\eta] \le \textstyle n^2 \tau(n, d, \eta).
%       \end{equation}
%       
%    We use tools from high-dimensional probability to find an appropriate function $\tau$ for a large class of predictors $g$, and show that the quantity $\textstyle n^2 \tau(n, d, \eta)$ vanishes for large $d.$ The proof is presented in the Appendix.
%\end{comment}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> related_work.tex <==
%!TEX root = main.tex
\section{Connections to related work}
\label{sec:related_work}

\textbf{Connections to the gradient variance}:
The gradient confusion condition has interesting connections to the variance of the gradients. If we assume bounded gradient variance $\sigma^2$, we can bound the gradient confusion parameter $\eta$ in terms of other quantities. For example, suppose the true gradient $g = g_1/2 + g_2/2.$ Then we can write: $| \langle g_1, g_2 \rangle | \leq \sigma^2 + \| g \|^2$, where all gradients are defined at the same $\mathbf{w}$.

However, in general one cannot bound the gradient variance in terms of the gradient confusion parameter.  As a counter-example, consider a problem with the following distribution on the gradients:  $\frac{1}{1-p}$ samples with gradient $\frac{1}{\epsilon}$ and $\frac{1}{p}$ samples with gradient $\epsilon$, where $p = \epsilon \to 0$. In this case, the gradients are positive, so gradient confusion $\eta = 0$. The mean of the gradients is given by $1+\epsilon (1-\epsilon)$, which remains bounded as $\epsilon\to0$. On the other hand, the variance (and thus the squared norm of the stochastic gradients) is unbounded ($O(1/\epsilon)$ as $\epsilon \rightarrow 0$). %While this is a contrived example, it does show why such a bound does not exist.
%
A consequence of this is that in theorems \ref{thm:cosine} and \ref{thm:nonconvex} in section \ref{sec:convergence}, the "noise term" (i.e., the second term in the RHS of the convergence bounds) does not depend on the learning rate in the general case. If gradients have unbounded variance, lowering the learning rate does not reduce the variance of the SGD updates, and thus does not reduce the noise term. This further indicates a regime of high gradient variance but low gradient confusion where SGD would converge faster than predicted by classical convergence rate results \citep{moulines2011non}.
%, needell2014stochastic}. 

In practice, typically the gradient variance is bounded. In this case, tighter convergence rate bounds in terms of $\eta$ are possible, which follow as simple corollaries from classical convergence bounds in terms of the gradient variance such as those in \cite{moulines2011non, needell2014stochastic}. The \emph{interpolation} and \emph{strong growth} conditions \cite{ma2017power, vaswani2018fast, srebro2010optimistic, schmidt2013fast}, are related to this. These conditions imply that the variance of the gradients at the minimizer is small. As shown above, this would imply that the gradient confusion is also small, leading to fast convergence of SGD.% This is also similar to the condition of the minimal risk being small \cite{srebro2010optimistic}.
%zhang2019stochastic}.

It is worth noting that the main contribution of this paper is to better understand how the network architecture impacts SGD. 
%In general, it is not tractable to prove the concentration bounds in sections \ref{sec:initialization} and \ref{sec:general_depth} using the covariance matrix of the gradients alone without further unrealistic assumptions, such as infinitely wide networks \citep{schoenholz2016deep}. 
A key contribution of this paper is to identify a suitable surrogate (i.e., the gradient confusion bound) to help study this relationship using new tight and clean bounds.

\textbf{Connections to gradient diversity:}
In \citet{yin2017gradient}, the authors define a property called \emph{gradient diversity}. This quantity is related to gradient confusion, but with important differences.
Gradient diversity also measures the degree to which individual gradients at different data samples are different from each other. However, the gradient diversity measure gets larger as the individual gradients become orthogonal to each other, and further increases as the gradients start pointing in opposite directions. In a large batch, higher gradient diversity is desirable, and this leads to improved convergence rates in distributed settings, as shown in Yin et al. (2017). 
On the other hand, gradient confusion between two individual gradients is zero unless the inner product between them is negative. %This makes gradient confusion useful for studying convergence of small minibatch SGD. This is because different possible SGD updates do not conflict with each other unless they are negatively correlated with each other.
%
This has important implications when we study the overparameterized setting. \citet{yin2017gradient} prove on 2-layer neural nets (and multi-layer linear neural nets) that gradient diversity \emph{increases} with increased width and decreased depth. Gradient diversity does not however distinguish between the cases where gradients become more orthogonal vs.~more negatively correlated. As we show in this paper, this can have very different effects on the convergence of SGD in overparameterized settings. Specifically, we show that increased width and decreased depth \emph{decreases} gradient confusion, and makes these networks easier to train. In fact, we see that the gradients become more orthogonal to each other in this case as shown in section \ref{sec:experiments}. Thus, we view our papers to be complementary to each other, providing insights about different issues (large batch distributed training vs.~small minibatch convergence).

\textbf{Other work on the impact of neural net structure:}
%
%Other works have also studied the impact of structured gradients on SGD. 
\citet{balduzzi2017shattered} study the effects of \emph{shattered gradients} at initialization for ReLU networks, which is when stochastic gradients at initialization become negatively correlated. The authors show how gradients get increasingly shattered with depth in ReLU networks.
%
\citet{hanin2018neural} shows that the variance of gradients in fully connected networks with ReLU activations is exponential in the sum of the reciprocals of the hidden layer widths at initialization. 
Further, \citet{hanin2018start} show that this sum of the reciprocals of the hidden layer widths determines the variance of the sizes of the activations at each layer during initialization. When this sum of reciprocals is too large, early training dynamics are very slow, suggesting the difficulties of starting training on deeper networks, as well as the benefits of increased width.

\textbf{Other work on SGD convergence:}
%
The convergence of SGD on over-parameterized models has received a lot of attention recently. \citet{arora2018optimization} study the behavior of SGD on over-parameterized problems, and show that SGD on over-parameterized linear neural nets is similar to applying a certain preconditioner while optimizing. This can sometimes lead to acceleration when overparameterizing by increasing the depth of linear neural networks. In this paper, we show that this property does not hold in general as depth keeps increasing.
There has recently also been interest in analyzing conditions under which SGD converges to global minimizers of overparameterized linear and non-linear neural networks. \citet{arora2018convergence} shows SGD converges  linearly to global minimizers for linear neural nets under certain conditions. \citet{du2018gradient, allen2018convergence, zou2018stochastic, brutzkus2017sgd} also show convergence to global minimizers of SGD for non-linear nets. While all these results require the network to be sufficiently wide, they represent an important step in the direction of better understanding optimization on neural nets. This paper complements these recent results by studying how low gradient confusion contributes to SGD's success on modern overparameterized neural nets.

%Our work differs from \cite{arora2018optimization} in that it studies a different mechanism of acceleration, and that we aim to establish a more direct relationship between width, depth, problem dimensionality, and the error floor of SGD convergence. 

% The behavior of SGD on over-parameterized problems was also studied in \cite{ma2017power, bassily2018exponential, vaswani2018fast, schmidt2013fast}, using an \emph{overfitting} condition observed for some overparameterized neural nets (particularly for convnets), where the minimizer returned by the optimizer simultaneously minimizes each individual data sample, to show fast convergence of SGD. In contrast, we aim to establish a more direct relationship between width, depth, problem dimensionality, and the error floor of SGD convergence.

%this study focuses on how and why network architecture choices affect convergence.

%The convergence of SGD on over-parameterized models have received quite a bit of interest recently. The authors of \cite{arora2018optimization} study the behavior of SGD on over-parameterized problems, and show that SGD on over-parameterized linear neural nets is similar to applying a certain preconditioner while optimizing.  
%\cite{ma2017power, bassily2018exponential, vaswani2018fast, schmidt2013fast} use an \emph{overfitting} condition observed for some overparameterized neural nets (particularly for convnets) where the minimizer returned by the optimizer simultaneously minimizes each individual data sample to show fast convergence of SGD. Our work studies a different mechanism of acceleration, and we focus on how and why network architecture choices affect convergence. 


%In \cite{yin2017gradient, chen2018effect}, the authors define a property called \emph{gradient diversity} that also measures the degree to which individual gradients at different data samples are different from each other. While this measure helps gain insights into large batch training, it does not distinguish between the cases where gradients are more orthogonal vs.~more negatively correlated. In this paper, we show that this can have very different effects on the convergence of SGD in overparameterized settings, and we view our works as complementary.

%This measure gets larger as the individual gradients become orthogonal to each other, and further increases as the gradients start pointing in opposite directions. In a large batch, higher gradient diversity is desirable, and this leads to improved convergence rates in distributed settings, as shown in \cite{yin2017gradient}. On the other hand, \emph{gradient confusion} between two individual gradients is 0 unless the inner product between them is negative. This is useful for studying convergence rates of small minibatch SGD since possible gradient updates do not conflict with each unless they are negatively correlated with each other. The choice of the definition of \emph{gradient diversity} in \cite{yin2017gradient} also has important implications when its behavior is studied in over-parameterized settings. \cite{chen2018effect} extends the work of \cite{yin2017gradient}, where the authors prove on 2-layer neural nets (and multi-layer linear neural nets) that gradient diversity increases with increased width and decreased depth. This does not however distinguish between the cases where gradients become more orthogonal vs.~more negatively correlated. In this paper, we show that this can have very different effects on the convergence of SGD. We show that increasing width and decreasing depth can have the effect of gradients becoming more orthogonal to each other, which in turn speeds up convergence of SGD, whereas decreasing width and increasing depth make gradients more negatively correlated, slowing down SGD's convergence.

%In this paper, we show that this can have very different effects on the convergence of SGD. We show that increasing width and decreasing depth can have the effect of gradients becoming more orthogonal to each other, which in turn speeds up convergence of SGD, whereas decreasing width and increasing depth make gradients more negatively correlated, slowing down SGD's convergence.


%There has recently also been interest in analyzing conditions under which SGD converges to global minimizers of overparameterized linear and non-linear neural networks  \cite{arora2018convergence, du2018gradient, allen2018convergence, zou2018stochastic, brutzkus2017sgd}. This paper complements these recent results by studying how one property, low gradient confusion, contributes to SGD's success on overparameterized neural nets.


